Understanding Reuse, Performance, and Hardware Cost of DNN Dataflows: A Data-Centric Approach Using MAESTRO

The data partitioning and scheduling strategies used by DNN accelerators to leverage reuse and perform staging are known as dataflow, and they directly impact the performance and energy efficiency of DNN accelerator designs. An accelerator microarchitecture dictates the dataflow(s) that can be employed to execute a layer or network. Selecting an optimal dataflow for a layer shape can have a large impact on utilization and energy efficiency, but there is a lack of understanding on the choices and consequences of dataflows, and of tools and methodologies to help architects explore the co-optimization design space. In this work, we first introduce a set of data-centric directives to concisely specify the space of DNN dataflows in a compilerfriendly form. We then show how these directives can be analyzed to infer various forms of reuse and to exploit them using hardware capabilities. We codify this analysis into an analytical cost model, MAESTRO (Modeling Accelerator Efficiency via Spatio-Temporal Reuse and Occupancy), that estimates various cost-benefit tradeoffs of a dataflow including execution time and energy efficiency for a DNN model and hardware configuration. We demonstrate the use of MAESTRO to drive a hardware design space exploration (DSE) experiment, which searches across 480M designs to identify 2.5M valid designs at an average rate of 0.17M designs per second, including Pareto-optimal throughput- and energy-optimized design points.

==> sections/02-Background-old.tex <==
\section{Background}
\label{sec:background}

\insertFigure{HWModel}{Abstract DNN accelerator architecture model which is pervasive in many state-of-the-art accelerators~\cite{eyeriss_isca, sharma2016high, parashar2017scnn, jouppi2017datacenter, aklaghi2018snapea}. %Network-on-chip includes all the interconnections such as inter-PE forwarding links which can be seen in a systolic array.
}


Although our approach can be applied to various DNN layers---CONV2D, fully-connected (FC), LSTM, separable convolution, and so on---we focus on CONV2D and its variants in this paper because convolutional neural networks (CNNs) are popular, and CONV2D accounts for more than 90\% of overall computation in CNNs~\cite{cong2014minimizing, eyeriss_isca}.
%
To understand the cost-benefit tradeoffs of various approaches to compute convolutions, we first introduce common DNN accelerator architectures, and discuss  core concepts related to  data reuse and dataflows.

\subsection{DNN Accelerators}
\label{subsec:DNNaccelerators}
DNN accelerators are specialized hardware to run DNN applications with high throughput and energy efficiency. As described in~\autoref{fig:HWModel}, most DNN accelerators employ hundreds of processing elements (PEs) to exploit inherent parallelism in DNN applications. PEs typically include scratchpad memories (L1) and ALUs that perform multiply-accumulate operations (MACs). To reduce energy- and time-consuming DRAM accesses, most DNN accelerators also include a shared  scratchpad buffer (L2) large enough to stage data to feed all the PEs. Shared L2 buffer and PEs are interconnected with a network-on-chip (NoC). Our approach supports a wide range of interconnect designs in the NoC module. For example, a systolic array could be represented as a 2D array that provides unidirectional links toward East and South. 
%
Depending on the hardware parameters selected, our approach can support architecture designs that can efficiently execute a wide range of DNN operations, including convolutions, because it enables exploiting not only parallelism but also data reuse via buffers and forwarding/multicasting NoCs. 

%However, dselecting an appropriate set of hardware parameters is a non-trivial task because of the complex relationship among hardware parameters, data flows, and the resulting data reuse patterns.
%To understand those aspects, we construct a concrete example of convolution in~\autoref{fig:7DConv} and describe the core concepts to understand the cost and benefits of various dataflow using the example with an emphasis on data movement and staging.

\subsection{Tensors in Convolution}
\label{subsec:tensors}

\insertFigure{7DConv_New}{An example convolutional layer with its dimensions and indexing are shown in (a), and a visualization of the convolution shown in (b). 
%Because input and output activation row/column indices are correlated, loop nest representation needs to choose either iterate over the input or output activation row/column dimensions.
%An input-centric and output-centric view of loop nests corresponding to the convolution is shown in (c) and (d) respectively. 
%(Bias terms and index bound checks are omitted for simplicity.) 
%A summary of the coupling among dimensions and data classes (tensors) are shown in (e), where a table entry with a check mark indicates that the dimension in the column is coupled with the data class in the row.}
}

We present an example of a 2D convolution in~\autoref{fig:7DConv_New} that involves seven data dimensions across three data structures: input/output activation and weight tensors.
Tensors in those three structures are coupled with seven dimensions in a complex manner.
For example, the row/column indices of output can be deduced using input row/column and filter row/column indices (i.e., an input-centric view of the convolution loop nest).
Also, the input channel index \texttt{c} appears in both filter and input activation, and the output channel \texttt{k} appears in both filter and output activation.
We call these dimensions {\it coupled} to these indices, as the position in the data space changes when the index is modified.
Because of these specific data access patterns, we can transform the loop nest to keep one of the data structures \emph{stationary} over a range of space or time (i.e., unchanged in a local buffer), which can significantly reduce global/local buffer access counts in DNN accelerators, as well as energy consumption by keeping local wires unchanging.
Such combinations of loop transformations and mappings to PEs are termed as {\em dataflows} in a prior work~\cite{eyeriss_isca}.
The work has categorized dataflows into three classes: weight-stationary, output-stationary, and input-stationary.
Although these classes provide a high-level characterization of strategies used when the work was published, the rapid rate of DNN accelerator development necessitates a more precise enumeration of the design space.
%and can be categorized into three classes - weight stationary, output stationary, and no-local-reuse - so as to cover a subset of dataflows that are frequently used in practice.

\begin{comment}
Different data movement schedule, tiling, and mapping of the tensors, which we define as dataflow in~\autoref{subsec:dataflowdescription}, lead to various data reuse patterns. Because data reuse is the prime behavior that accelerators exploit to deliver high throughput and energy efficiency, the cost model, \tool, also models it as the first-order target behavior. \tool classifies data reuse in three classes based on their reuse span in time and space (PEs). We discuss the taxonomy in the following subsection.
\end{comment}


\subsection{Data Reuse Taxonomy}
\label{subsec:datareuse}

%\input{DataReuse_table}

\insertFigure{DataReuse}{An operational example of a weight-stationary style accelerator over four PEs. For simplicity, input/output channels and batch are omitted. A 2x2 kernel (R=2, S=2) is used in this example.}


%%\insertWideTableFigure{DataReuseTable}{A summary of three data reuse types in DNN accelerators. Exploiting data reuse opportunities requires costs as listed in this table.}

We broaden the taxonomy of dataflows by observing that data reuse originates from two behaviors of DNN accelerators over time and space - multicasting (input tensors) and reduction (output tensors).
%

\betterparagraph{Multicasting} Spatial multicasting reads a data point from a buffer only once, spatially replicates the data point via wires, and delivers the data point to multiple spatial destinations (i.e., PEs), which reduces expensive remote buffer accesses and saves energy.
%
Likewise, temporal multicasting also reads a data point from a large remote buffer only once, temporally replicates the data point via a smaller local buffer, and delivers the data point to multiple temporal destinations (i.e., different time instances) at the same PE, which also reduces expensive remote buffer accesses and saves energy.
%

\betterparagraph{Reduction} Spatial reduction accumulates partial outputs from multiple spatial sources and spatially accumulates them via multiple compute units (e.g., an adder tree).
%
Similarly, temporal reduction accumulates partial outputs from multiple temporal sources (i.e., partial sums computed at different time) and temporally accumulates them via an accumulation register or buffer (e.g., accumulation buffer in TPU~\cite{jouppi2017datacenter}).

When multicasting or reduction temporally occurs, it provides temporal reuse opportunity, and vice versa.
%
For example, ~\autoref{fig:DataReuse} shows an operational example of weight-stationary dataflow style run on four PEs.
%
We can observe that $W_{1}$ is multicasted across time, which is temporal multicasting, $I_{1}$ is multicasted across space (PEs), which is spatial multicasting, and $P_{3\_0}$ is reduced across space and time.
%
That is, the example accelerator temporally reuses $W_{1}$ and spatially reuses $I_{1}$ and $P_{3\_0}$.
%
%However, to actually exploit the data reuse opportunities, the accelerator 
%With appropriate hardware supports, we can covert such data reuse opportunities into reald data reuse.


\begin{comment}

The purpose of staging is to keep data points in a local buffer to reuse them in the future, multicasting is to simultaneously send the same data points to multiple PEs to amortize the cost of buffer access, and forwarding to send data points to adjacent PEs so that they can be reused in future iterations.
%
We define staging as \textit{temporal} reuse and multicasting and forwarding as \textit{spatial} reuse. We categorize both of multicasting and forwarding as spatial reuse because their data reuse is across space (PEs), and they are hardware implementation choices that materialize spatial reuse opportunity in a different manner.

%each of those reuse behaviors as \textit{temporal}, \textit{spatial}, and \textit{spatio-temporal} reuse respectively. 

\autoref{fig:DataReuse} shows a timeline of a row-stationary accelerator (logical PE version ~\cite{eyeriss_isca}) with four PEs. 
%We show example data reuse opportunity for three data reuse classes we introduced. 
%shows how data points are reused over time and across PEs in an example 2-dimensional convolution. 
%We can observe how data points are reused over time and across PEs in a 2-dimensional convolution example in Fig. 5.  FIg. 5(a) shows a partial sums computation.  Fig. 5 (b) highlights examples of three data reuse classes we discuss next.
~\autoref{fig:DataReuse} (b) highlights examples of (1) temporal, (2) spatial (multicasting), and (3) another spatial (reduction) data reuse. The {\tt weight} data value W1 is used at cycle 0 in PE3, and used again at cycle 2 in the same PE, which is \textit{temporal reuse}. Input data value I1 is used at cycle 0 across PE2 and PE1, which is \textit{spatial reuse}. The partial sum P$_{3\_1}$ is accumulated at cycle 3 in PE0 but generated by PE3 at cycle 2, which is spatial reuse across time (\textit{spatio-temporal}). Note that any given architecture may or may not exploit all of these opportunities. %Although a dataflow provides data reuse opportunities, if the target accelerator lacks components to support them, the reuse opportunity cannot be exploited. For example, if the buffer size in a PE is not sufficient, the PE needs to overwrite data points, which could be temporally reused, and refetch them from the shared buffer when the PE needs them again. Therefore, all the reuse implied by dataflows are reuse opportunities. 
%We define those reuse opportunities and discuss how they are implied in~\autoref{table:DataReuseTable}.

As shown in~\autoref{fig:DataReuse} (b), we can observe that the data reuse occurs either across time or space (across PEs).
%
Within each data reuse, two reuse styles, multicasting and reduction, exist.
%
Multicasting is reuse for input tensors (input activation and filter), which indicates that the same data points are replicated over time or space.
%
Reduction is reuse for output tensors (output activation), which indicates that the same output is replicated over time or space.
%
That is, if the dataflow is legal (does not perform redundant computation), partial sums for the replicated output are accumulate over time or space.
%
Note that such replication of data points across time and space implies \texttt{data reuse opportunities} not actual data reuse.
%
To materialize such data reuse opportunities, appropriate hardware support is required, which we discuss in~\autoref{subsec:hardware_implementation}.

%\autoref{table:DataReuseOpportunities} summarizes the three types of data reuses in DNN accelerators, and also presents opportunities and implications for those data reuses. Each data reuse requires specific conditions to be met in the dataflow (or, loop nest structure). Temporal reuse is mainly related to the loop order and buffers, multicasting-based spatial reuse is mainly related to the coupling of a data structure dimensions to the spatially mapped (or, iterated in a {\tt parallel-for}) dimension and NoC structure, and forwarding-based spatio-temporal reuse is related to all of the aspects in temporal/spatial reuse. That is, loop nest structures need to be organized in a specific style to reveal data reuse opportunities with a proper accelerator. Such restructured loop nests correspond to various dataflows.

\end{comment}


\subsection{From Loop Nest to Dataflow}
\label{subsec:dataflowdescription}
%\vspace{-2mm}

\insertWideFigure{Unrolled1DConvExample}{An example 1D convolution and an example output-stationary dataflow on the convolution. We represent the dataflow (b) in loop nest and (c) data-centric directives. In (c), gray boxes represent omittable descriptions, which can be inferred (upper gray box) or does not affect the data reuse over PEs (lower gray box).  (d) shows an abbreviated form of the dataflow description in data-centric directives. (e) and (f) show resulting mapping on PEs and iteration space, whose dots correspond to computation (or, partial sums).}

%\TK{Change title. Say that we define dataflow to be ...}
Dataflows are often expressed as \emph{loop nests}, a syntax that resembles a simple imperative programming language with explicit parallelism, as presented in Eyeriss v2~\cite{chen2018eyeriss}. 
%The mechanisms used by DNN accelerators to leverage data reuse, or dataflow, can be understood as a combination of loop transformations including tiling and mapping loops onto PEs. Dataflows are often expressed as {\emph loop nests} with explicit annotation of parallelism, as presented in Eyeriss v2~\cite{chen2018eyeriss}. We term this approach as a compute-centric approach because the loop variable directly specify the computation ID, not data indices (Note that some data indices do not match with computation IDs; e.g., input indices y'+r and x'+s in ~\autoref{fig:7DConv} (d))
We term the loop nest notation a \emph{compute-centric} representation since the data movement is implicit from the loop order and the explicit parallelism specified by the programmer.
%
The loop order dictates the schedule (or, ordering) of computations, the explicit annotation of loops with {\tt parallel-for} captures parallelism, and the combination of loop ordering, tiling and parallelism enables data reuse. 
% The example in ~\autoref{fig:DataMappingExample} (a) describing a version of row-stationary dataflow~\cite{eyeriss_isca} has two {\tt parallel-for} with a specific loop order that constructs the row-stationary dataflow. Also, loop \texttt{c} in the original loop nest in ~\autoref{fig:7DConv} (d) is tiled into \texttt{c1} and \texttt{c0} and separated by \texttt{parallel\_for  y'} in~\autoref{fig:DataMappingExample} (a) to implement tiling. Upon those components, the loop order in the loop nest, i.e., ({\tt n->k1->c1->y'->k0->c0->x'->r->s}) implicitly guides data movement within accelerators across multiple levels of memory hierarchy, which influences data reuses.
Therefore, architects started to explore optimized loop nests encompassing all of the three aspects; loop order, parallelism, and tiling. For example, Eyeriss v2~\cite{chen2018eyeriss} describes its dataflow in a 22-dimensional loop nest.

% Since parallelism and loop order are the first class entities in a compute-centric (loop-nest) representation, inferring accurate data movement in the accelerator and then developing cost models to precisely estimating efficiency is challenging. 
%is challenging because the loop nest is an abstraction for software developers that lack the mapping information on PEs, which includes the number of PEs, the tile mapping on PEs, PE clustering (e.g., 2D array), and so on. Hence, inferring cost and benefits of dataflows in a loop nest representation is also challenging. 

% This motivates us to explore alternative intermediate representation (IR) of dataflows that focus on data, a data-centric representation of dataflows where data movement and organization are being the first class entities.

Compute-centric representation (i.e., loop-nest notation) including the polyhedral model has been a huge help to compilers in estimating reuses in guiding optimal loop transformations for both parallelism and locality~\cite{DBLP:journals/ibmrd/Sarkar97,DBLP:conf/ispass/SarkarM00,DBLP:conf/cc/ShirakoSFPRSS12,Wolf:1991:DLO:113445.113449,Bondhugula:2008:PAP:1375581.1375595,DBLP:conf/sc/PouchetBBCRS10,Shirako:2014:OWM:2683593.2683626}.
%
Those works provide sufficiently accurate cost estimations to drive a series loop transformation in a compiler.
%
However, they do not precisely model data reuse so computing throughput and energy-efficiency with high accuracy is challenging for those works.
%
%This past work provides estimates that are sufficient to drive selection of loop transformations in compilers, but they are limited in their ability to estimate reuse precisely enough to obtain accurate estimates of throughput and energy-efficiency. 
%
Bao et al.~\cite{Bao:2017:AMC:3177123.3158120} developed an analytical model to accurately estimate cache behavior (thereby computing reuses) for a class of affine programs that can be precisely analyzed by a polyhedral model at compile time. 
%
However, they use heavyweight linear-algebra frameworks within the polyhedral model to compute reuse, thereby making it impractical to use these techniques on large real applications.
%
Also, it is very challenging for the polyhedral-based frameworks to compute reuse arising from array subscripts involving non-affine expressions or complex subscripts, such as modulus operations which are common in strided convolutions.
%

In addition, although there exists a body of past compiler work that performs reuse analysis on sequential programs~\cite{DBLP:journals/ibmrd/Sarkar97,DBLP:conf/ispass/SarkarM00,DBLP:conf/cc/ShirakoSFPRSS12,Wolf:1991:DLO:113445.113449,Bondhugula:2008:PAP:1375581.1375595,DBLP:conf/sc/PouchetBBCRS10,Shirako:2014:OWM:2683593.2683626,Bao:2017:AMC:3177123.3158120}, they lack the ability to analyze loop nests with explicit parallelism while DNN dataflows often contain multiple levels of parallelism.
%
Also, those past works did not consider spatial reuse(which does not refer to spatial locality in cache-based architectures but data reuse via wires or acress PEs) that leverages multicasting and reduction support of accelerators, which plays a key role in estimating the overall throughput and energy efficiency of spatial DNN accelerators.
%

Such limitations and challenges motivate us to explore an alternative intermediate representation (IR) of dataflows, a \emph{data-centric} representation where data movement and organization are first-class entities.
%
Since data movement is explicit in the data-centric representation, our analytical model becomes simpler and relatively faster as there is no need to leverage heavyweight linear-algebra frameworks to precisely estimate data movement / reuse behavior.



==> sections/03-Dataflow-old.tex <==

\section{Describing Dataflows}
\label{sec:dataflow-IR}

\insertWideFigure{Dataflow_Examples}{The impact of directive order, spatial/temporal maps, tile sizes, and clustering.}

In this section, we introduce our {\em data-centric} representation to represent various accelerator dataflows. We illustrate four key directives of our representation: 1) spatial map, 2) temporal map, 3) data movement order, and 4) clusters. We use 1D convolution (shown in~\autoref{}(a)) as a pedagogical example. 
%
Then, we briefly discuss the construction of dataflows using our representation, and then explain various hardware implementation choices for supporting a wide range of data-reuses across space, time, and space-time.% viable through our data-centric directives.  

\subsection{Data-Centric Representation}
We define the dataflow of an accelerator design to consist of two major aspects -- 1) The schedule of DNN computations (e.g., choice of loop transformations) across time for exploiting a wide range of reuses, and 2) The mapping of the DNN computations across PEs for parallelism.
%
To explicitly describe above key aspects of dataflows, we propose a data-centric representation that clearly describes data mappings and movement behavior, unlike compute-centric representations in the loop nest form which imply them.
%
The representation is based on four key components that are briefly discussed below with examples. \\

\noindent
{\bf 1) Spatial Map(size, offset) X} specifies a distribution of the dimension X of a data class across PEs, where {\tt size} refers to the number of indices mapped in the dimension {\tt X} to each PE, and {\tt offset} describes the shift in the starting indices of {\tt X} across consecutive PEs. 
%
For example, {\tt SpatialMap(1,1) X'} of  mapping A in~\autoref{fig:Dataflow_Examples} (where {\tt X'} refers to the first dimension of output data class), spatially distributes indices of the {\tt X'} dimension with a chunk size of one (derived from the {\tt size} parameter) across PEs with an offset of one (derived from the {\tt offset} parameter).
%
This spatial data distribution can be viewed from the data space of output data class in the same column of mapping A in~\autoref{fig:Dataflow_Examples}.
%
If the number of PEs is not sufficient to cover all indices of the dimension mapped, then the mapping is folded over time across the same set of PEs. 
%
Also, if {\tt offset} value is smaller than {\tt size} value, then there will be an overlap of indices across consecutive PEs, and this is useful in describing mappings on X and Y in input-centric notation because their iteration space is skewed.  \\

\noindent
{\bf 2) Temporal Map(size, offset) X} specifies a distribution of the dimension X of a data class across time steps in a PE, and also the mapped chunk of dimension indices is the same across PEs in a time step. 
%
Similar to spatial map, {\tt size} refers to the number of indices mapped in the dimension {\tt X} to each PE, and {\tt offset} describes the shift in the starting indices of {\tt X} across consecutive time steps in a PE. 
%
For example, {\tt TemporalMap(1,1)S} of mapping A in~\autoref{fig:Dataflow_Examples} (where {\tt S} refers to the first dimension of filter weight data class), distributes indices of the {\tt S} dimension with a chunk size of one (derived from {\tt size} parameter) across time steps with an offset of one (derived from {\tt offset} parameter).
%
This temporal distribution can be viewed from the data space of the filter weight data class in the same column of mapping A in~\autoref{fig:Dataflow_Examples}.
%
Since all PEs get same data indices corresponding to a temporally mapped dimension, this may create opportunities for {\em spatial reuse}, i.e., spatially reusing the same data values across PEs in a time step. \\

\noindent
{\bf 3) Data Movement Order: } The sequence of spatial and temporal maps in the dataflow specification dictate the order of data movement, i.e., change in the data mappings to PEs across time. 
%
A change in the order can result in an entirely different stationary behavior. 
%
For example, the sequence of directives in mapping A in~\autoref{fig:Dataflow_Examples}, i.e., spatial map on {\tt X'} followed by the temporal map on {\tt S}, indicates that all data indices of S should be explored before working on the next chunk of {\tt X'} indices. 
%
This order results in temporally reusing values of data corresponding to  {\tt X'}  indices, i.e., partial sums, for all indices of {\tt S}, leading to output stationary dataflow. 
%
This behavior can be observed from the iteration space for the mapping A in~\autoref{fig:Dataflow_Examples}.
%
Now, if the order of directives is interchanged, i.e., temporal map on {\tt S} followed by spatial map on {\tt X'} shown in mapping B in~\autoref{fig:Dataflow_Examples}, results in weight-stationary dataflow, because PEs can temporally reuse values of data corresponding to {\tt S} indices, i.e., weight values, for all indices of {\tt X'}  before going to next chunk of {\tt S} indices.
%
Similarly, mappings C and D in~\autoref{fig:Dataflow_Examples} shows the spatial distribution on {\tt S} instead {\tt X'}, and also the impact of data movement order on temporal reuses leading to different stationary dataflows. 

In all of the mappings from A-D in~\autoref{fig:Dataflow_Examples}, the mapping sizes (first argument) of all mappings are one -- resulting in either no temporal reuse (e.g., partial output sums in case of mapping B) or full temporal reuse (e.g., input feature map in case of mapping C). 
%
Increasing the map size of the spatial or temporal maps can help in presenting opportunities for partial temporal reuse, which can capture convolutional reuse in CNN layers. 
%
For example, the spatial map corresponding to the {\tt S} dimension in mapping E in~\autoref{fig:Dataflow_Examples} helps in exploiting partial temporal reuse of input data across time steps.\\



\noindent
{\bf 4) Cluster (size, type)}:  As can be seen from the data movement orders in mappings from A-E in~\autoref{fig:Dataflow_Examples}, data mappings related to a map in outer position gets updated after full exploration of a map in inner position. 
%
For example,  spatial map on {\tt S} followed by the temporal map on {\tt X'} in Mapping E, indicates that all data indices of {\tt X'} should be entirely explored before working on the next chunk of {\tt S} indices.
%
This inherent assumption can limit certain dataflow behaviors where one might be interested in simultaneously exploiting spatial distribution of more than one data dimensions.

We introduced the {\em Cluster} directive as a mean to support the simultaneous spatial distribution of multiple data dimensions. 
%
The cluster directive works by logically grouping multiple PE's or multiple sub-clusters of {\tt size} parameter, e.g., cluster(3) in mapping F in~\autoref{fig:Dataflow_Examples} groups available PEs in groups of 3, resulting in two clusters.
%
The advantage of clusters directive is that mappings specified before the directive are applied across the logical clusters resulted from grouping, and mappings specified after the directive are applied inside the logical cluster. 
%
With this intuition, one can specify spatial maps after and before the cluster to explore multi-dimensional spatial distribution. 
%
An example of this can be seen in mapping F in~\autoref{fig:Dataflow_Examples}, where {\tt X'} dimension is spatially distributed across clusters, and {\tt S} dimension is spatially distributed within the cluster. 
%
We use the cluster directive to represent popular row-stationary dataflow in Eyeriss~\cite{eyeriss_isca} since it involves the spatial distribution of R and Y dimensions simultaneously, and also NVDLA dataflow~\cite{nvdla} which involves the spatial distribution of K and C dimensions. 
\PC{TODO: Didn't talk about type parameter of the cluster?}

 Another advantage of our cluster directive is that its notion of grouping multiple PEs can represent coarse-grained PEs in our abstract hardware model, such as SIMD units~\cite{song2016cbrain} and matrix tensor accelerators like GPU Tensor cores. 


With the above four key components of our 
data-centric representation, all possible aspects of dataflow, i.e., scheduling and mapping, can be represented elegantly. 
%
For example, the loop-nest version of a dataflow involving multi-level tiling for the 1D convolution is shown in~\autoref{}(b), and its corresponding data-centric representation with our directives is shown in~\autoref{}(c). 
%
Currently, data-centric representation of a dataflow could be either autogenerated by our framework from the correct description of a loop nest version of the dataflow, or manually written. 


%{\bf Construction of dataflows:}

% {\bf Implication on hardware structures}: Data reuses resulting from dataflows poses a requirement of hardware structures, for e.g., temporal reuses require a temporary buffer such as L1 to store data temporarily. 
% %
% Also, Fanout network on chip or store-and-forward structures are required to exploit spatial reuse from hardware. 





%\insertFigure{Dataflow_Tilesize}{The impact of mapping (tile) size on dataflow}

%\insertWideTableFigure{ReuseTable}{A|B means one of A and B.}

\input{tables/HW_Implication_table.tex}

\insertTableFigure{HW_Impl_choices}{Hardware Implementation Choices for supporting spatial and temporal reuse. Note - by {\it temporal multicast}, we refer to {\it stationary} buffers from which the same data is read over time.}


%%\insertHugeFigure{DataMappingExample}{A deep dive of data mapping into an example of Eyeriss~\cite{eyeriss_isca} dataflow. We use color to indicate changes in the data index and corresponding mapping pragma. Time step in (d), (e), and (f) is the unit temporal iteration, which is the fundamental time concept in the \tool framework. We discuss it in ~\autoref{subsubsec:unit_iterations}. }


%\subsection{Dataflow to Reuse to Hardware Implications}
%\label{subsec:reuse_implications}

%\TK{Table on implications of dataflow on reuse and HW}

% \subsection{Construction of Dataflows}
% \label{subsec:dataflow_legality}

% The first and foremost principle in constructing dataflows is that data mappings corresponding to data dimensions of all data classes should be specified. 
% %
% If 


% The dataflow description directives are flexible that users can specify any data mapping following a uniform pattern for each dimension.
% %
% However, like the flexibility of programming languages allow users to write buggy code, dataflow directives allow users to specify illegal dataflows.
% %
% Legal dataflows must meet the following conditions:

% \colonparagraph{Bound condition} Bound condition is the first requirement that prohibits mappings of non-existing indices.
% %
% For example, in the example layer presented in~\autoref{fig:7DConv}, the number of output channels (K) is four.
% %
% Therefore, TemporalMap(5,5) K is an illegal mapping directive because the mapping size (five) in the directive exceeds the bound of K dimension (four).

% \colonparagraph{Coverage condition} Coverage condition requires the data mapping to cover all the pairs of operands (inputs and weights in CNNs) to generate the desired outputs.
% %
% For example, in the dataflow in~\autoref{fig:DataMappingExample}, if we replace the second directive, TemporalMap(2,2) K, to TemporalMap(2,4) K, the dataflow becomes illegal because the dataflow does not cover entire output channels (K).
% %
% \tool prints out warning messages when the dataflow does not cover all the pairs of operands assuming CNNs as the target program.
% %
% However, in some cases such as stride larger than one in a CNN or dilated convolutions can intentionally drop some data points to implement their functionality.
% %
% Therefore, users need to carefully review the dataflow when they use \tool to model such cases.

% \colonparagraph{No redundancy condition} No redundancy condition prevents redundant data mapping that produces the same output as previously mapped data points.
% %
% That is, once a set of operands are mapped on a PE, all the computation using the operands need to be done at the PE.
% %
% For example, in the dataflow in~\autoref{fig:DataMappingExample}, if we replace the third directive, TemporalMap(3,3) C, with TemporalMap(2,1) C, the dataflow becomes an illegal one because a redundant input channel is mapped along two temporal iterations of C.


\subsection{Hardware Implementation Choices for Data Reuses from Dataflows} 



==> sections/03-DataflowDescription.tex <==

\section{Describing Dataflows}
\label{sec:dataflow-IR}
%\TK{ i updated the section title} \HK{I updated it again because we changed our positioning strategy}

\TK{TODO - Precisely define dataflow}

To explicitly describe key aspects of dataflows, we propose a {\em data-centric} IR that clearly describes (1) data iteration schedule, (2) data tiling, and (3) data mapping on PEs, unlike computer-centric representations in the loop nest form imply them.
%
The IR is based on three data-centric dataflow directives - spatial map, temporal map, and cluster - that describe how each dimension of data iterates over time (iterations) and space (PEs), how large a mapping over each iteration is for each dimension, and how we organize the granularity of the mapping over space (PE clustering).
%
We discuss the syntax and semantics of those three directives in the following subsection.

\subsection{Data-centric Dataflow Directives}
\label{subsec:dataflow-directives}

%%\insertWideFigure{DirectiveExample}{Operating examples of three dataflow directives. For cluster and map directive examples, the number of PEs is 12 and 4, respectively.}

%\insertWideTableFigure{DirectiveTable}{The syntax and semantics of dataflow directives. For cluster and map directive examples, the number of PEs is 12 and 4, respectively.}

Because data in DNN accelerators are high dimensional tensors, we take the divide-and-conquer strategy: we describe the tiling and mapping of each dimension and stack them to represent the tiling and mapping of entire data in a data class (input/weight/output), as presented in~\autoref{fig:DataMappingExample} (b).
%
We represent the data iteration order using the order of dataflow directives for each dimension, similar to the loop order in the compute-centric representation.
%
Although the concept of schedule implied by order of data/compute dimension is similar, two directives, temporal and spatial map, in the proposed directives innately encapsulate the tiling and mapping over time/space.%, unlike compute-centric version requires complex loop transformations.
%
Also, the other directive, cluster, enables manipulating the spatial granularity of mapping.
%
We discuss the syntax and semantics of each directive next.

\TK{Move these to a table form:}

\subsubsection{Cluster: Dimensionality in PE array}
\label{subsubsec:cluster}

\colonparagraph{Syntax} \texttt{Cluster(size, type)}, where size is integer, and type is either L (logical) or P (physical)

\colonparagraph{Semantics} The base clusters at the inner-most loop directive are logical PEs. Cluster directive is processed from the innermost one, and it bundles \texttt{size} sub-clusters at the level \texttt{cluster} is specified to construct superclusters that becomes unit spatial dimension for directives outer than the \texttt{cluster}. 
If the \texttt{type} is physical, the super cluster constructed by the \texttt{cluster} becomes the unit physical compute unit, or physical PE.
If no physical cluster is defined, the logical PEs are treated as physical PEs.

\colonparagraph{Implication} \texttt{cluster} enables to describe mapping over multi-dimensional processing element array with static/dynamic grouping of PEs.
For example, Eyeriss~\cite{eyeriss_isca} has a 2D PE array and constructs a dynamic cluster over rows to cover the row dimension of a sliding window.
Two \texttt{cluster} directives can be used to describe such clustering.

\colonparagraph{Example} In the example in~\autoref{fig:DirectiveExample} (c), two \texttt{cluster} directives are defined in the order of \texttt{cluster (3,P)} and \texttt{cluster (2,L)}. Because cluster is constructed from the inner-most level, \texttt{cluster(2,L)} first operates on 12 logical PEs and generates level 1 clusters that contain two logical PEs each. 
Other directives between \texttt{cluster(3,P)} and \texttt{clsuter(2,L)} operates on the level 1 clusters., %using them as the unit spatial dimension.
\texttt{cluster(3,P)} groups three level 1 clusters and construct two level 2 clusters.
All directives above \texttt{cluster(3,P)} operate on the level 2 cluster.
Because of the type \texttt{P} specified in \texttt{cluster(3,P)}, level 2 clusters are mapped on a physical PE.
Logical PEs within a level 2 cluster, or a physical PE, potentially operate as vector lanes of ALUs depending on the vector lane of the target hardware.

\subsubsection{Temporal Map: Tiling and mapping over time}
\label{subsubsec:temporal-map}

\colonparagraph{Syntax} \texttt{TemporalMap (size, offset) x}, where size and offset are integers and \texttt{x} is a data dimension.

\colonparagraph{Semantics} \texttt{TemporalMap} directives specify (1) the number of elements mapped in a dimension x (``size") and (2) how the mapping move in the next iteration of x (offset) to all of the sub-clusters.

\colonparagraph{Implication} \texttt{TemporalMap} maps the same set of elements in a dimension to all the sub-clusters. 
It expresses data tiling using \texttt{size} and tile iteration rule over time using \texttt{offset}. 

\colonparagraph{Example} \texttt{TemporalMap(3,1) X} in~\autoref{fig:DirectiveExample} (a) indicates that three elements in X dimension is mapped in each iteration, and the mapping shifts by one in the next iteration.
%
That is, the mapped x over time is (0,1,2), (1,2,3), (2,3,4), and so on.
%

\subsubsection{Spatial Map: Tiling and mapping over space}
\label{subsubsec:spatial-map}

\colonparagraph{Syntax} \texttt{Spatial (size, offset) x}, where size and offset are integers, and x is a data dimension.

\colonparagraph{Semantics} \texttt{SpatialMap} directives specify (1) (1) the number of elements mapped in a dimension x (``size") and (2) how the mapping move in the next cluster (offset). 
When the size of the spatial dimension (number of sub-clusters) is not sufficient at the level \texttt{SpatialMap} is specified, the spatial mapping is folded over time.

\colonparagraph{Implication} \texttt{SpatialMap} maps different sets of elements in a dimension to sub-clusters.
It expresses data tiling using \texttt{size} and tile iteration rule over space using \texttt{offset}. 

\colonparagraph{Example} \texttt{SpatialMap(3,1) Y} in~\autoref{fig:DirectiveExample} (b) indicates that three elements in Y dimension is mapped on each cluster (in this example, logical PEs) and the mapped elements shift by one over space (PEs).
%
That is, the mapped y on each PE is as follows: PE0 <= (0,1,2), PE1 <= (1,2,3), PE2 <= (2,3,4) .., PE5 <= (5,6,7).
%
Because the number of PEs is not sufficient to cover entire Y dimension, the mapping is folded over time.


\subsection{Data Movement Order}
\label{subsec:data_movement_order}

\TK{Need some text}
The schedule of tile iterations, or data movement order, is one of the key aspects of dataflow, which determines temporal reuse.
%
The dimension in the outer-most loop in loop nest-based representation and outer-most directive in data-centric directive-based representation changes in the slowest rate among all the data dimensions, and vice-versa for the dimension in the inner-most loop or directive.
%
That is, by comparing the relative positions of loop or directive, we can identify which dimension changes relatively faster or slower in a given dataflow description.
%

To infer stationary data from the directive order, we need to consider another aspect, dimension coupling with data classes.
%
We presented how each of seven dimensions correlate to each data class (Input feature map, filter weight, and output feature map) in~\autoref{fig:7DConv}.
%
If the dimension whose mapping is changing does not couple with a data class, the data class is stationary between two mappings (original and changed mapping), or over time.
%
For example, if only output channel mapping is updated between two sets of mappings, input feature map does not change between two mappings since input feature map does not have output channel dimension in its data dimension.
%


%Although the insight is simple, actual analysis is not trivial because mappings over multiple dimensions can change at the same time, some of mappings over dimensions might be the first iteration, which requires full data load, and some of mappings over dimenisons might be on the edge of the data, which results in smaller mapping than the mapping size described in a directive (e.g., if the layer has only three input channels (C), temporalMap(10,10) C, need to map three input channels, not ten, to prevent out-of-bound error).


\subsection{Dataflow Playground}
\label{subsec:dataflow_playground}
In this subsection, we illustrate our data centric representation of dataflows with examples.

{\bf Spatial and temporal map}: These mappings are used to specify data distributions of dimensions of data classes across PEs and time. A spatial map corresponding to a dimension of a data class specifies a distribution of the dimension across PEs. For example, {\tt SpatialMap(1,1)X'} of  mapping A in~\autoref{fig:Dataflow_Examples} (where {\tt X'} refers to the first dimension of output data class), spatially distributes indices of the {\tt X'} dimension with a chunk size of one (derived from {\tt size} argument) across PEs. The distribution can be viewed from the data space of output feature map in the same column of mapping A in~\autoref{fig:Dataflow_Examples}, where PEs get consecutive indices of {\tt X'} in a given time step. 

%
Similarly, temporal map specifies a distribution of the dimension across time steps in a given PE, and also the mapped chunk of dimension indices is the same across PEs in a time step. For example, {\tt TemporalMap(1,1)S} of mapping A in~\autoref{fig:Dataflow_Examples} (where {\tt S} refers to the first dimension of filter weight data class),  distributes a chunk of size one index of the {\tt S} across time steps  in a given PE. The distribution can be viewed from the data space of filter weight, where all PEs get the same chunk of indices of {\tt S} across PEs in a given time step, but consecutive indices in later time steps. 
Since all PEs get same data values corresponding to a temporally mapped dimension, this creates opportunities for spatial reuse, i.e., spatially reusing the same data values across PEs in a time step.

{\bf Data movement order}: The sequence of spatial and temporal maps in the dataflow specification dictate the order of data movement, i.e., change in the data mappings to PEs across time. A change in the order can result in an entirely different stationary behavior. For example, the sequence of directives in mapping A in~\autoref{fig:Dataflow_Examples}, i.e., spatial map on {\tt X'} followed by the temporal map on {\tt S}, indicates that all data indices of S should be explored before working on the next chunk of {\tt X'} indices. This order results in temporally reusing values of data corresponding to  {\tt X'}  indices, i.e., partial sums, for all its chunk of {\tt S}, leading to output stationary dataflow. This behavior can be observed from the iteration space for the mapping A in~\autoref{fig:Dataflow_Examples}. Now, if the order of directives is interchanged, i.e., temporal map on {\tt S} followed by spatial map on {\tt X'} shown in mapping B in~\autoref{fig:Dataflow_Examples}, results in weight-stationary dataflow because PEs can temporally reuse values of data corresponding to {\tt S} indices, i.e., weight values, for all its chunk of {\tt X'} indices before going to next chunk of {\tt S} indices.
%
Similarly, mappings C and D in~\autoref{fig:Dataflow_Examples} shows the spatial distribution on {\tt S} instead {\tt X'}, and also the impact of data movement order on temporal reuses leading to different stationary dataflows. 
\PC{Talk about spatio-temporal reuse in the mappings as well}


{\bf Impact of non-unit map sizes in spatial and temporal maps}: In all of the mappings from A-D in~\autoref{fig:Dataflow_Examples}, the mapping sizes (first argument) of all mappings are one -- resulting in either no temporal reuse (e.g., partial output sums in case of mapping B) or full temporal reuse (e.g., input feature map in case of mapping C). Increasing the map size of the spatial or temporal maps can help in presenting opportunities for partial temporal reuse, which can capture convolutional reuse in CNN layers. For example, the spatial map corresponding to the {\tt S} dimension in mapping E in~\autoref{fig:Dataflow_Examples} helps in exploiting partial temporal reuse of input data across time steps.


{\bf Exploiting multi-dimensional spatial distributions}:
As can be seen from the data movement orders in mappings from A-E in~\autoref{fig:Dataflow_Examples}, data mappings related to an outer map gets updated after full exploration of the inner map. For example,  spatial map on {\tt S} followed by the temporal map on {\tt X'} in Mapping E, indicates that all data indices of {\tt X'} should be explored completely before working on the next chunk of {\tt S} indices. This inherent assumption can limit certain dataflow behaviors where one might be interested in simultaneously exploiting spatial distribution of more than one data dimensions. So, we introduced {\em Cluster} directive as a mean to support simultaneous spatial distribution of multiple data dimensions, and the cluster directive works by logically grouping multiple PE's or multiple sub-clusters, e.g., cluster(3) in mapping F in~\autoref{fig:Dataflow_Examples} groups available PEs in groups of 3, resulting in two clusters.
%
The advantage of clusters directive is that mappings specified before the directive are applied across the logical clusters resulted from grouping, and mappings specified after the directive are applied inside the logical cluster. With this intuition, one can specify spatial maps after and before the cluster to explore multi-dimensional spatial distribution. An example of this can be seen in mapping F in~\autoref{fig:Dataflow_Examples}, where {\tt X'} dimension is spatially distributed across clusters, and {\tt S} dimension is spatially distributed within the cluster. We use the cluster directive to represent popular row-stationary dataflow in Eyeriss~\cite{eyeriss_isca} since it involves the spatial distribution of R and Y dimensions simultaneously, and also NVDLA dataflow~\cite{nvdla} which involves the spatial distribution of K and C dimensions. 

{\bf Support for coarse-grained PEs}:
Another advantage of our cluster directive is that its notion of grouping multiple PEs can represent coarse-grained PEs in our abstract hardware model, such as SIMD units~\cite{song2016cbrain} and matrix tensor accelerators like GPU Tensor cores. By representing such coarse-grained PEs using our cluster directive, our cost model to estimate energy and throughput estimates doesn't need to be modified.


% {\bf Implication on hardware structures}: Data reuses resulting from dataflows poses a requirement of hardware structures, for e.g., temporal reuses require a temporary buffer such as L1 to store data temporarily. 
% %
% Also, Fanout network on chip or store-and-forward structures are required to exploit spatial reuse from hardware. 



\insertWideFigure{Dataflow_Examples}{The impact of directive order, spatial/temporal maps, tile sizes, and clustering.}

%\insertFigure{Dataflow_Tilesize}{The impact of mapping (tile) size on dataflow}

%\insertWideTableFigure{ReuseTable}{A|B means one of A and B.}

\input{tables/HW_Implication_table.tex}

\insertTableFigure{HW_Impl_choices}{Hardware Implementation Choices for supporting spatial and temporal reuse. Note - by {\it temporal multicast}, we refer to {\it stationary} buffers from which the same data is read over time.}

\TK{TODO: Examples of dataflows with implications on reuse etc. Impact of spatial vs temporal, impact of ordering, impact of size parameter, and impact of clustering. Hyoukjun owns this right now.}

%%\insertHugeFigure{DataMappingExample}{A deep dive of data mapping into an example of Eyeriss~\cite{eyeriss_isca} dataflow. We use color to indicate changes in the data index and corresponding mapping pragma. Time step in (d), (e), and (f) is the unit temporal iteration, which is the fundamental time concept in the \tool framework. We discuss it in ~\autoref{subsubsec:unit_iterations}. }


%\subsection{Dataflow to Reuse to Hardware Implications}
%\label{subsec:reuse_implications}

%\TK{Table on implications of dataflow on reuse and HW}

\subsection{Legal Dataflows}
\label{subsec:dataflow_legality}

The dataflow description directives are flexible that users can specify any data mapping following a uniform pattern for each dimension.
%
However, like the flexibility of programming languages allow users to write buggy code, dataflow directives allow users to specify illegal dataflows.
%
Legal dataflows must meet the following conditions:

\colonparagraph{Bound condition} Bound condition is the first requirement that prohibits mappings of non-existing indices.
%
For example, in the example layer presented in~\autoref{fig:7DConv}, the number of output channels (K) is four.
%
Therefore, TemporalMap(5,5) K is an illegal mapping directive because the mapping size (five) in the directive exceeds the bound of K dimension (four).

\colonparagraph{Coverage condition} Coverage condition requires the data mapping to cover all the pairs of operands (inputs and weights in CNNs) to generate the desired outputs.
%
For example, in the dataflow in~\autoref{fig:DataMappingExample}, if we replace the second directive, TemporalMap(2,2) K, to TemporalMap(2,4) K, the dataflow becomes illegal because the dataflow does not cover entire output channels (K).
%
\tool prints out warning messages when the dataflow does not cover all the pairs of operands assuming CNNs as the target program.
%
However, in some cases such as stride larger than one in a CNN or dilated convolutions can intentionally drop some data points to implement their functionality.
%
Therefore, users need to carefully review the dataflow when they use \tool to model such cases.

\colonparagraph{No redundancy condition} No redundancy condition prevents redundant data mapping that produces the same output as previously mapped data points.
%
That is, once a set of operands are mapped on a PE, all the computation using the operands need to be done at the PE.
%
For example, in the dataflow in~\autoref{fig:DataMappingExample}, if we replace the third directive, TemporalMap(3,3) C, with TemporalMap(2,1) C, the dataflow becomes an illegal one because a redundant input channel is mapped along two temporal iterations of C.



==> sections/03-backup.tex <==

We discussed the syntax and semantics of dataflow directives we propose and their implication.
%
To represent a full dataflow, directives must be defined over all the sub-dimensions of each data; seven dimensions introduced in~\autoref{fig:7DConv} (a).
%
~\autoref{fig:DataMappingExample} (b) describes a row-stationary dataflow~\cite{eyeriss_isca} described in our directives over the layer defined in~\autoref{fig:7DConv} (b).
%
The dataflow is equivalent to the dataflow implied by ~\autoref{fig:DataMappingExample} (a).
%
Using this example, we discuss how to determine the directives for each dimension and organize them to represent the row-stationary dataflow described in~\autoref{fig:DataMappingExample}.

\colonparagraph{Clustering PEs} The row-stationary dataflow treats R x S logical PEs (R/S: filter row/column size) as a cluster and maps an outputs row on each cluster.
%
For simplicity, we allocate logical PEs as physical PEs and map S elements of the filter column dimension (unrolling S dimension) on each PE, which corresponds to \texttt{TemporalMap(3,3) S} in~\autoref{fig:DataMappingExample} (b).
%
Because the logical PEs are physical PEs, the cluster directive has the type of "logical."
%
Also, because the size of the R dimension is three in the target layer, the cluster size is three.
%
Therefore, we obtain a cluster directive \texttt{Cluster(3,L)} as described in~\autoref{fig:DataMappingExample} (b)
%
Note that clusters might introduce additional directives (at maximum, number of cluster directives extra "map"s for a dimension) because a SpatialMap directive defined over a cluster does not indicate how the mapped elements are distributed within a cluster.
%
For example, ~\autoref{fig:DataMappingExample} (b) contains two SpatialMap directives for Y dimension in each cluster level.

\colonparagraph{Tiling Tensors} In the row-stationary dataflow, PEs in a cluster compute partial sums for output, and each PE is responsible for a row in the sliding window generating S partial sums.
%
Therefore, for each PE, one R element, three S elements (unrolled), and one Y element need to be mapped.
%
We can determine the number of X elements to be mapped, but we select the minimum size (three; following S dimension size).
%
For input/output channels, we tile into two and three elements (different sizes) to show how tiling works in the example.
%
For input batch, we use the batch size of one as the row-stationary accelerator, Eyeriss, also processes one batch.
%
Therefore, the tile size of each dimension in a PE is as follows: (N:1, K:2, C:3, Y:1, X:3, R:1, S:3).
%

\colonparagraph{Scheduling data iteration} Because the S dimension is unrolled in each PE, the map directive for S dimension is placed at the bottom.
%
Over S dimension, because each PE generates partial sums for a filter row, R and Y elements need to be distributed over the logical PEs.
%
To prevent duplicated partial sums, we specify SpatialMap of R and Y.
%TemporalMap is invalid because it maps the same set of R and Y elements that lead to duplicated partial sums.
%
%Therefore, SpatialMap of R and Y needs to be specified.
%
The order of R and Y can be any because R dimension is unrolled in a cluster.
%
%That is, mapped elements in the R dimension do not change over Y distribution iterations in both ordering (Y->R and R->Y).
%
Although all the clusters operate on different output rows, they iterate over the output column (X dimension) in the same manner as presented in~\autoref{fig:DataMappingExample} (c), which requires a TemporalMap on X.
%
Another SpatialMap of Y over X dimension needs to be specified to allocate different output rows over clusters.
%
%Note that this SpatialMap of Y operates over clusters while the previous one operates over PEs in a cluster.
%
C and K dimensions can be in any order above the last SpatialMap of Y.
%
We place C dimension first for output reuse and use TemporalMap to prevent redundant data mapping.
% because partial sums need to accumulate also along input channels (C), while partial sums do not accumulate along output channels (K).
%
%We use TemporalMap of C and K because spatially mapping C and K in this dataflow results in uncovered partial sums.
%
Finally, we place the batch at the top because different batch can be interpreted as another run over a different input activation tensor.
%
Therefore, we obtain the data iteration schedule as follows: (tMap N-> tMap K-> tMap C-> sMap Y-> tMap X (Cluster) sMap Y-> sMap R-> tMap S, where tMap and sMap are TemporalMap and SpatialMap directives)

\colonparagraph{Constructing stacked directives} We aggregate the constructed cluster, tiles, and schedules in previous steps to describe a full dataflow.
To determine the offset, we consider if the dataflow requires overlapped data points between temporal/spatial iterations or not.
%
For tMap N, tMap K, and tMap C, we select the same offset as the tile size because they should not be overlapped.
%
In contrast, we select an offset of one for sMap Y and tMap X to describe overlapping between adjacent sliding windows.
%
%For example, in~\autoref{fig:DataMappingExample} (c), mapped input data points in time step 0 and 1 has overlapped data points because sliding window shifted by one while the mapping size is three.
%
Within a cluster, all of the sMap Y, sMap R, and tMap S have offset values the same as tile size to prevent redundant data mapping. % because overlapped data points are not expected, resulting in redundant partial sum generation.
%
Applying those offset values, we finally obtain the dataflow described in~\autoref{fig:DataMappingExample} (b).

%\squishlist
%    \item{Bound condition: The mapping size should not exceed the index bound of a dimension}
%    \item{Coverage condition: A dataflow needs to cover all the combination of data points required for producing outputs.}
%    \item{No redundancy condition: The combinations of data points should not be replicated over time or PEs.}
%\squishend

==> sections/04-backup.tex <==
\section{Quantitative Dataflow Analysis}
\label{sec:framework}

%\insertFigure{HighLevelAlgorithm}{A high-level overview of algorithms in \tool.}

\insertFigure{PerformanceCostAnalysisEngine}{A high-level overview of algorithms in performance and cost analysis engines.}

\insertWideFigure{AnalysisFramework}{An overview of \tool's analysis framework. For simplicity, we omit components other than analysis engines.}

In this section, we present our approach to quantitatively estimating runtime and energy efficiency of dataflows on a target DNN model and hardware configuration.
%
Based on the approach, we implement an analysis framework, \tool, which consists of five engines: tensor, cluster, data reuse, performance analysis, and cost analysis.
%
~\autoref{fig:AnalysisFramework} provides a high-level overview of the five engines.
%
In the interest of space, we only discuss high-level algorithms without edge case handling, multiple layers, and multiple cluster levels.
%
For details, we present them in our open-source repository\footnote{https://github.com/georgia-tech-synergy-lab/MAESTRO}.

\subsection{Tensor Analysis}
\label{subsec:tensor_analysis}

As described in~\autoref{fig:AnalysisFramework}, the tensor analysis engine identifies dimension coupling for each tensor based on specified layer operations.
%
For example, in depth-wise convolutions, output channel is not coupled with output-channel dimension, but the input channel.
%
Note that depth-wise convolution can be understood as either this way or eliminating input channel dimension (C).
%
We select this convention because it aligns with \tool's input-centric cost model.
%
\tool allows users to specify tensors with arbitrary dimension coupling, and such coupling relationship is input to the rest of engines, which provides generality to \tool.
%


%\insertFigure{Preprocessing}{Preprocessing procedures of PE cluster hierarchy analysis engine.}

\subsection{Cluster Analysis}
\label{subsec:pe_cluster_hierarchy_analysis}

A PE cluster refers to a group of PEs that processes one or more data dimensions in parallel, which is specified by the \Cluster directive.
%
~\autoref{fig:HighLevelAlgorithm} (b) shows a brief description of the Cluster Analysis (CLA) engine.
The CLA engine analyzes a given dataflow description written in dataflow directives to identify the number of sub-clusters in each cluster level, extract cluster dataflow directives and data dimensions for each cluster level, and augment the given dataflow descriptions for missing directives, stride handling, and so on.
%
%cluster levels and identifies the number of active unit clusters (i.e., PEs) to run a given dataflow (~\autoref{fig:Preprocessing} (a)), extracts dataflow and sub-dimesion sizes for each cluster level(~\autoref{fig:Preprocessing} (b)), mapping size of each dimension in each cluster level(~\autoref{fig:Preprocessing} (c)), possible data iteraetion positions(~\autoref{fig:Preprocessing} (d)), and augments the data-centric directives to handle omitted directives, input- and output-centric notation conversion, stride handling, and so on (~\autoref{fig:Preprocessing} (e)).
%

\begin{comment}
\betterparagraph{Cluster size analysis} The CHA engine first evaluates cluster sizes from the lower-most cluster level, which is the bottom-most cluster in a data-centric dataflow representation, to the top and calculates the total number of PEs, or unit clusters.
%
Based on the total number of unit clusters (PEs) specified by users, the CHA engine infers the minimum number of active unit clusters to run an input dataflow.
%
For example, in~\autoref{fig:EyerissDeepDive} (b), \Cluster(3,L) directive exists, which implies we need at least three unit clusters to form the lowest level cluster and run this dataflow.
%
If the number of PEs is not sufficient (e.g., 2 in this example), \tool outputs an error message and terminates.
%
If a user specifies 168 PEs, $168 \div 3 = 56$ lowest-level clusters are constructed.
%
When the number of PEs is not even divisible by the number of unit clusters in the second top-most cluster, the remainder PEs are inactive.
%

\betterparagraph{Cluster dataflow extraction} The CHA engine traverses through each directive in the data-centric representation and extracts dataflow directives for each cluster level with dimension size information.
%
The data dimension size needs to be updated for each cluster level because a data dimension size in a cluster is the mapping size of its upper cluster (For the top-most cluster, it is the same as the layer dimension).
%
That is, at a non top-most cluster level, the size of each data dimension is inherited from the mapping size of the corresponding dimension in the upper level cluster.
%
For example, in~\autoref{fig:EyerissDeepDive} (b) has two cluster levels.
%
In the lower cluster level, the size of data dimension Y is 3 because \tMap(3,1) Y is specified in the upper cluster.


\betterparagraph{Dataflow Directive Augmentation} At each cluster level, mapping directives over all the dimensions need to be specified.
%
If no directive is specified on a data dimension, \tool automatically inserts \tMap (\textit{dimension size}, \textit{dimension size}), which effectively fully unrolls the corresponding dimension.
%
Also, the CHA engine internally converts output-centric notation, a data-centric dataflow representation that uses output activation dimensions (X' and Y') instead of input activation dimensions (X and Y).
%
In addition to the discussed augmentation, the CHA engine also updates the directives to reflect stride size, which enables users to specify the dataflow without tuning directives for strides in the same way a user deals with layers with unit stride size.
%

\end{comment}

%\insertFigure{ReuseAnalysis}{Some selected core algorithms in data reuse analysis engine.}

\subsection{Data Reuse Analysis}
\label{subsec:data_reuse_analysis}

~\autoref{fig:AnalysisFramework} (b) includes a high-level description of analysis in data reuse analysis (DR) engine.
%
DR engine identifies the amount of temporal and spatial reuse across adjacent time steps, which is the data iteration corresponding to the inner-most non-temporally/spatially unrolled mapping directive.
%

\begin{comment}

To compute the exact amount of data reuse, we first analyze reuse opportunities by computing 
the number of temporally and spatially reused data points in each data structure during an accelerator run.
%
The Data Reuse Analysis (DRA) engine identifies such reuse opportunities 
%
For simplicity, we discuss reuse analysis within a single cluster because we can repeatedly apply the same method for each cluster level in multi-level cluster cases.
%
To focus on core ideas, we omit various edge cases when the data dimension size to map is smaller than the mapping size (temporal edge), the number of sub-clusters in a cluster level (spatial edge), or both of those (spatio-temporal edge) although they are all dealt in the DRA engine.
%
~\autoref{fig:ReuseAnalysis} presents core algorithms in DRA engine.
%
\betterparagraph{Prime Changing Dimension}
When a data mapping moves at each unit time step, one of the dimensions proceed and rest of them either resets to the initial position or remain stationary.
%
This is similar to the behavior of loop variables in a loop nest.
%
For example, loop variable x in ~\autoref{fig:7DConv_New} (c) increments only if the iteration moves to the next step when (r,s) = (2,2) and they are updated to (r,s) = (0,0).
%
When such an update occurs, all the loop variable above loop x remains stationary.
%
In this example, the dimension x is the prime changing dimension.
%

In data mapping iterations, we can observe the same behavior; a data dimension $\alpha$ coupled with a directive in the middle of dataflow directives is updated only if all the dimensions coupled with directives below the directive on $\alpha$.
%
The inner-most data dimension neither initialized to its initial position nor fully unrolled is the prime changing dimension, which can be computed as presented in~\autoref{fig:ReuseAnalysis}.
%
Unrolled directives are \tMap with mapping size larger than its corresponding dimension size or \sMap with the spatial coverage (mapping size + (number of sub-clusters) $times$ offset; when mapping size > offset).
%
The prime changing dimension is critical to compute temporal reuse.

\betterparagraph{Temporal Reuse Analysis}
%Temporal reuse occurs when a set of data points are replicated in mappings of adjacent time steps.
%
%We use the inner-most data iteration as the unit time step in our analysis, which corresponds the inner-most non-unrolled mapping directive.
%
%Unrolled directives are \tMap with mapping size larger than its corresponding dimension size or \sMap with the spatial coverage (mapping size + (number of sub-clusters) $times$ offset; when mapping size > offset).
%
%
To compute the temporal reuse, the DRA engine tracks the changes in data mapping of each tensor across every possible two adjacent unit time steps, as shown in~\autoref{fig:ReuseAnalysis} (b).
%
%For example, in Mapping A presented in~\autoref{fig:Dataflow_Examples}, the inner-most iteration is "\tMap (1,1) S."
%
%When the mapping changes from the unit time step 0 to 1 (t=0 to t=1 in the example), only mapped {\tt S} changes.
%
%Because the filter is coupled with {\tt S} dimension, the filter mapping changes over those two temporal iterations.
%
%However, the output does not change because it is not coupled with {\tt S} dimension, indicating full temporal reuse of outputs.
%
%This approach is valid when a mapping changes only over the dimension of inner-most dataflow directive.
%
%However, data dimension iterations also periodically reset to the initial position proceeding the iteration of upper data directives. This is similar to a loop iteration variable in a loop nest, which resets to zero and increments loop variable(s) based on upper loops.
%

The amount of spatial reuse depends on where the data mapping traverses in the entire data space, which we term as data dimension iteration status.
%
For each dimension, only three data dimension iteration states exist: \texttt{Init}, \texttt{Steady}, \texttt{Edge}. 
%
\texttt{Init} refers to the first position of the data dimension iteration, which corresponds to the initial value of a loop variable in a loop nest.
%
\texttt{Steady} refers to all the non-init data iteration positions except edge cases.
%
\texttt{Edge} refers to the last data iteration position when the remaining dimension size is less than the mapping size of a \tMap or the spatial coverage of \sMap.
%

\HK{Algorithms to compute iteration cases and number of case occurrence is not added yet.}
The DRA engine analyzes the dataflow and data dimension sizes and extracts all the possible combinations of iteration positions for each data dimension, which results in a maximum of $3^7$ cases (not likely to occur in practice unless an extremely inefficient mapping is selected).
%
The DRA engine identifies how the mapping is updated for each tensor in each case, the number of case occurrences, and the amount of temporal data reuse during execution.

\betterparagraph{Spatial Reuse Analysis}
The key observation for spatial reuse analysis is that reuse analysis of temporal and spatial map is identical but spatial reuse needs to consider spatial steps (analogous to the concept of time steps) in a certain granularity, or number of sub-clusters (in the lowest cluster level, PEs) at the corresponding cluster level.
%
That is, the DRA engine computes the spatial reuse in the same way as temporal reuse analysis, but groups up the number of sub-clusters spatial steps (time steps in the temporal reuse case) and identifies the reuse in this granularity, which makes the spatial reuse analysis presented in~\autoref{fig:ReuseAnalysis} (c) a super set of temporal reuse analysis in~\autoref{fig:ReuseAnalysis} (b).
%
%When the same data sets are mapped across all the spatial steps, it implies full spatial reuse or a broadcasting opportunity.
%
%When some sets of data are mapped across some of the spatial steps, it implies partial spatial reuse or a multicasting opportunity.
%

\end{comment}

\subsection{Performance Analysis}
\label{subsec:performance-analysis}

~\autoref{fig:AnalysisFramework} (a) presents a high-level overview of performance and cost analysis engine, and~\autoref{fig:PerformanceCostAnalysisEngine} shows high-level algorithm of the performance analysis (PA) engine.
%
Utilizing the reuse information computed in DR engine, the performance analysis (PA) engine computes the runtime for all the possible cases based on the data dimension and dataflow.
%
The computed runtime is multiplied with the number of each case's occurrences, and accumulated to compute the total runtime.
%
The runtime of a DNN accelerator consists of communication delay (L2 to L1, L1 to L2, local forwarding) and computation delay in each PE, which are directly related to the accelerator's hardware parameters.
%
PA engine considers the double buffering when it computes the outstanding delay (the worst case delay of communication/computation delay) that directly contributes to the runtime.
%

%The Performance Analysis (PA) engine computes all of the delays considering hardware parameters, dataflow, and data reuse.
%

To estimate communication delays, \tool relies on its analytical network-on-chip (NoC) model, which is a pipe model similar to other analytic models~\cite{parashar2019timeloop}.
%
The pipe model utilizes two parameters, the pipe width (bandwidth) and length (average delay), to estimate the communication delay via NoC.
%
The model incorporates a pipelining effect as many packet-switching NoCs have similar behavior.
%
Various combinations of the bandwidth and average delay enables to model NoC structures with reasonable accuracy.
%
For example, Eyeriss~\cite{eyeriss_isca} has a two-level hierarchical bus with a dedicated channel for three data structures (inputs, weights outputs).
%
Therefore, a bandwidth of 3X properly models the top level buffer.
%
The average latency depends on implementation details; users should choose an appropriate value considering implementation details (e.g., both of ingress/egress buffers or one of them might exist in a bus implementation, which adds one cycle delay each).
%
For more complicated NoC architectures, users should select bisection bandwidth and average latency considering uniform communication to all the PEs from a global buffer.
%
For example, a $N \times N$ 2D mesh network with the injection point at one of the corners, the bisection bandwidth is $N$ and the average latency is $N$.
%
Assuming that the user has access to the NoC implementation information, the NoC model is precise when the NoC is a bus or a crossbar. 

\begin{comment}

\betterparagraph{Accelerator Model}
\tool receives the following parameters listed in~\autoref{fig:HWModel} as inputs: number of PEs, vector processing width per PE, interconnect latency, buffer sizes, and bandwidth.
%
The hardware model is a hierarchy of PE clusters with buffers at the highest (L2 global scratch pad) and lowest (L1 local scratch pad) and interconnection between adjacent PE cluster levels.
%
~\autoref{fig:HWModel} shows the simplest case of the hardware model that has no additional PE cluster level.
%
In multi-cluster level cases, the network-on-chip and PE array structure in~\autoref{fig:HWModel} is replicated.


\betterparagraph{NoC Model}
\tool employs an analytic NoC model based on a pipe model, similar to other analytic models~\cite{parashar2019timeloop}.
%
The pipe model utilizes two parameters, the pipe width (bandwidth) and length (average delay), to estimate the communication delay via NoC.
%
The model incorporates a pipelining effect as many packet-switching NoCs have similar behavior.
%
Various combinations of the bandwidth and average delay enables to model NoC structures with reasonable accuracy.
%
For example, Eyeriss~\cite{eyeriss_isca} has a two-level hierarchical bus with a dedicated channel for three data structures (inputs, weights outputs).
%
Therefore, a bandwidth of 3X properly models the top level buffer.
%
The average latency depends on implementation details; users should choose an appropriate value considering implementation details (e.g., both of ingress/egress buffers or one of them might exist in a bus implementation, which adds one cycle delay each).
%
For more complicated NoC architectures, users should select bisection bandwidth and average latency considering uniform communication to all the PEs from a global buffer.
%
For example, a $N \times N$ 2D mesh network with the injection point at one of the corners, the bisection bandwidth is $N$ and the average latency is $N$.
%
Assuming that the user has access to the NoC implementation information, the NoC model is precise when the NoC is a bus or a crossbar. 

\betterparagraph{Runtime Estimation} 
To evaluate the runtime, we perform a worst-case analysis to estimate the delay of each unit time step at each cluster level.
%
That is, we compare computation, L2-to-L1 communication, L1-to-L2 communication, and PE to PE forwarding delays and select the longest delay as the computation delay of the corresponding cluster level since the worst case delay is the outstanding delay observed from the upper level cluster.
%
The PA engine applies double-buffering and latency-hiding based on a user-specified parameter to enable users to explore the tradeoff between buffer size and performance.
%

To compute both computation and communication delay, the PA engine identifies the total number of computations for each sub-cluster (or PE in the lowest cluster level), the amount of \texttt{unique} data of each tensor across adjacent unit time steps in each data dimension iteration case.
%
In the lowest level cluster, the computation delay is the worst case number of computations for a PE divided by the vector width of the datapath in each PE.
%
The L2 to L1 communication delay is the amount of unique input/filter data divided by the NoC bandwidth plus tail delay of NoC pipeline.
%
We apply the same method to the L1 to L2 communication delay except that we use the amount of unique output data.
%
For multi-level cluster cases, we compute from the lowest level cluster and apply the outstanding delay as the computation delay of the upper level cluster.

\betterparagraph{Bottleneck Analysis} The PA engine also reports the bottleneck delay of each iteration case via an output log file.
%
Users can review the output file and identify the source of the bottleneck and try updating either hardware parameters or dataflow to eliminate the bottleneck.
\end{comment}

\subsection{Cost Analysis}
\label{subsec:cost-analysis}

~\autoref{fig:PerformanceCostAnalysisEngine} describes how the cost analysis (CA) engine computes the number of buffer accesses and estimates the buffer size requirements for each tensor, considering data reuse computed in DR engine and data iteration cases.
%
Utilizing the access counts and the number of MAC operation information, \tool computes the energy cost.
%
\tool includes an energy model based on those activity counts and Cacti~\cite{muralimanohar2009cacti} simulation, which can be replaced by any other energy model based on such activity counts (e.g., Accelergy~\cite{iccad_2019_accelergy}).

\begin{comment}

The major cost of DNN accelerators is data movement~\cite{eyeriss_isca} so modeling movement and reuse is the key to DNN accelerator cost estimation, which is the prime target of the Cost Analysis (CA) engine's analysis.

\betterparagraph{Buffer Access and Computation Counts} The CA engine estimates the activity counts of buffer accesses at each hierarchy and computations, which is the basis of the energy estimation of \tool.
%
To precisely estimate the activity counts, the CA engine combines information reported by other engines including PE cluster hierarchy information reported by the CHA engine, cluster dataflow information reported by the CHA engine, and the data reuse information reported by the DRA engine.
%
The CA engine counts all the buffer accesses within each cluster level and all the mapped unique data points across buffer hierarchies, which includes data reuse.

\betterparagraph{Buffer Size Requirements} The CA engine estimates the buffer size requirement by identifying the worst-case mapping size of each buffer hierarchy and prints out warning messages if the user-specified buffer size is not sufficient to support the target dataflow.
%
The mapping size of each tensor is the product of all the mapping sizes of coupled dimensions to the tensor.
%
The total buffer size requirements are the sum of mapping size of all the tensors.
%
Depending the dataflow, the CA engine also reserves buffer space for partial sums in global buffers.
\end{comment}

%
%Also, buffer sizing at various levels of the memory hierarchy is a crucial component in DNN accelerator design as it restricts the appropriate tile sizes and temporal reuse opportunities afforded by any dataflow.
%
%DNN accelerators today spend significant area and energy for buffers~\cite{pellauer2019buffets}.
%Therefore, precisely estimating the amount of buffer required to support an input dataflow is crucial for DNN accelerator designers. Also, global/local buffer access counts are directly related to the energy consumption because their unbalanced energy consumption and their analysis is as follows.

%\colonparagraph{Determining Buffer Size} \tool defines the minimum local scratchpad (L1) size to support a dataflow as the tile size mapped on each PE in each unit temporal iteration (and doubles it for double buffering). %Note that we double the tile size to model double buffering.
%For shared buffer (L2) size requirement, \tool computes the unique data points across the PE array within two temporal iterations (and doubles it). Depending on the dataflow, \tool also accounts for storage required for partial sums to prevent
%redundant DRAM accesses.

%\colonparagraph{Buffer Access Counts} For local scratchpad (L1), \tool identifies the number of data points to generate all the partial sums within a tile mapped on a PE in each unit iteration. This number contributes to both of L1 read and write. The number of output tensor data points is counted as L1 writes. Those numbers are multiplied by the total number of unit temporal iterations.
%
%For shared buffer (L2), \tool identifies the number of unique data points mapped over entire PE array in each unit temporal iteration. \tool multiplies the number with the number of entire unit temporal iterations and add up them to L2 read counts. We count the number of data points read from DRAM as L2 write counts. %
%For both of L1 and L2, partial sum accumulation may increase L2 access counts when the input dataflow generates partial outputs from each unit spatial iteration. 
%Also, note that the buffer analysis engine also considers all the realistic aspects discussed in~\autoref{subsec:performance-analysis-engine}. In particular, data reuse converts high L2/DRAM counts into affordable L1 access counts, effectively reducing energy consumption.

\subsection{Complex Dataflow Analysis}
\label{subsec:complex_dataflow_analysis}

\betterparagraph{Multi-cluster Analysis}
As we discussed in this section so far, multi-cluster cases can be split into single-cluster cases with the data dimension size set as the mapping size of the corresponding mapping directive in the upper cluster.
%
The outstanding delay of a cluster level becomes the computation delay of the next cluster level above.
%
To handle various edge cases that affects all the lower cluster levels, \tool recursively performs performance and cost analysis, as illustrated in~\autoref{fig:AnalysisFramework}. 
%
In the recursive analysis, the base case is the inner-most cluster whose sub-clusters are actual PEs.
%
Although \tool performs recursion, the complexity is not high because the number of PE cluster levels are typically two or three.
%
In summary, the multi-cluster analysis is recursive cost analysis whose base case is the lowest level cluster that has unit clusters (i.e., PEs) as sub-clusters.
%
To deal with edge cases, each of the edge cases at each cluster level also needs to be recursively processed.
%
However, in most cases, we observe the number of edge cases across cluster levels are less than 20, which is still in a tractable scale.

\betterparagraph{Other DNNs}
Although we used dense convolution as examples for simplicity, \tool can model a variety of layers (LSTM hidden layer, pooling, fully-connected, transposed convolution, and so on) based on the generality of the data-centric approach.
%
Our data-centric approach supports all the operations represented as the loop nest with two input tensors and one output tensor wherein all the tensor indices are coupled in only one or two data dimensions in affine functions.
%
\tool also can model uniformly distributed sparsity for any supported dataflow. 
%
Support for more complex statistical sparsity distributions is future work.

\subsection{Model Validation}
\label{subsec:validation}

\insertFigure{Validation}{Runtime model validation against MAERI~\cite{kwon2018maeri} RTL simulation with 64 PEs and Eyeriss~\cite{chen2017eyeriss_issc} runtime reported in the paper with 168 PEs.}

We validated \tool's performance model against RTL simulations of two accelerators - MAERI~\cite{kwon2018maeri} and Eyeriss~\cite{chen2017eyeriss_issc} when running VGG16 and AlexNet respectively\footnote{MAERI RTL is open-source. For Eyeriss, we use the reported runtime for AlexNet because detailed mapping parameters are described for only AlexNet in the paper.}.
%
\autoref{fig:Validation} shows that the runtime estimated by \tool are within 3.9\% absolute error of the cycle-accurate RTL simulation and reported processing delay~\cite{chen2017eyeriss_issc} in average.
%

%As we show later in our evaluations, the power of \tool is to explore the HW implementation design-space for an existing accelerator (e.g., DLA~\cite{nvdla} or Eyeriss~\cite{chen2017eyeriss_issc}) and determine the appropriate configuration given a target area/power/performance/energy target.

==> sections/05-MAESTRO.tex <==


\subsection{The MAESTRO Tool}

\AP{Cut / Shorten}

%\subsection{Input Specification}
%\label{subsec:DFSL}

%\insertFigure{DFSLExample}{An example of input specification to \tool that describes VGG16~\cite{VGGnet} DNN model, dataflows of each layer of the model, and hardware description of a target accelerator. }

The input to \tool consists of a DNN model, hardware description, and dataflows described in data-centric directives discussed in~\autoref{sec:dataflow-IR}. 
%
~\autoref{fig:DFSLExample} shows a sample specification of the VGG16 model as an input to the framework. 
%
Each layer of the model also includes a description of dataflow using a sequence of our data-centric directives discussed in~\autoref{subsec:dataflow-directives}.
%
Also, a hardware description of target accelerator such as the number of PEs, sizes of L1/L2 buffers and bandwidth of NoC are specified. 
%
\tool supports a wide range of layers including convolutional, pooling, fully-connected, and so on.
%
\tool also models sparse DNN layers via specifying a percentage of sparsity for each data class assuming a uniform distribution of zeros.


\subsection{Outputs}
\label{subsec:maestro_outputs}

%\insertFigure{OutputCapture}{An example output of MAESTRO.}

\autoref{fig:OutputCapture} shows an example output of MAESTRO analysis.
%
MAESTRO prints out (TBA)
%
MAESTRO also generates csv files that contains cost information of valid design points explored during design space exploration when a user activates DSE.


\TK{Add a snapshot or table showing outputs of MAESTRO.}

\begin{comment}

\section{Design Space Exploration}
\label{sec:dse}

Using \tool, we implement a hardware design space exploration (DSE) tool that searches five hardware parameters (the number of PEs, L1/L2 buffer sizes, NoC bandwidth, and vector width in ALUs) optimized for either energy efficiency, throughput, or throughput per Watt within given hardware area and power constraint.
%
The DSE tool receives layer dimensions, dataflow description, hardware area, and power constraints, and the area and power of building blocks synthesized with the target technology as inputs.
%
For the cost of building blocks, we implement FP multiplier and adder, bus, bus arbiter, global and local scratch pad in RTL and synthesis them using 28nm standard cell and SRAM library. For bus and arbiter cost, we fit the costs into a linear and quadratic model using regression because the bus cost increases linearly and the arbiter (matrix arbiter) cost increases in a quadratic manner.
%
Users can specify one of the three optimization targets: runtime (throughput), energy, or run time-energy product.
%

The DSE tool searches entire legal search spaces within given constraints and outputs the optimal hardware parameters it searched and corresponding \tool analysis results (buffer access counts, estimated execution time, and others).
%
It also reveals the bottleneck point (L2 to L1 or L1 to L2 communication, or computation) that hinders to achieve the roof-line performance so that users can adjust the constraints and dataflows to mitigate the bottleneck. 
%
Users also can replace the area and power information of building blocks using the building block RTL we provide and their technology library to perform DSE using a different technology.
%
We present case studies using DSE tool in~\autoref{subsec:dse_eval}.

\end{comment}


\subsection{Supported Dataflows}
\label{subsec:dfcasestudy}

%Although we used dense convolution as examples for simplicity, 
\tool can model a variety of layers (LSTM hidden layer, pooling, fully-connected, separable convolution, and so on) thanks to the generality of our data-centric approach that specifies a mapping of input tensors.
%; any operations in a layer require two operands, or data, and data-centric approach specifies the mapping of data points (operands). 
%
%Users can specify various layers by specifying layer type using dataflow specification language (DFSL) we introduce in~\autoref{subsec:DFSL}.
%
For LSTM hidden layer, we use the input width (dimension X) to specify the input size to the hidden layer, input channel (dimension C) to specify different gates.
%
For convolution with stride, pooling layer, and transposed convolution, users need to specify the stride, pooling size, and expansion factor, respectively.
%
%The DFSL syntax allows users to specify them (e.g., changing Type in one of the layers in~\autoref{fig:DFSLExample} into POOL, TRCONV and so on).
%
\tool also models uniformly distributed sparsity for any supported dataflow.
%because \tool model performs static analysis that is not able to handle d. % which is available for static analysis.
%
%To support the estimation upon real data with sparsity, we need a dynamic component that inspects the real distribution of zeros in input data, which is out of the scope of this work.
%

%\tool 
\tool does not support programs with non-affine indices because most DNNs have only affine data indices.
%However, DNNs have only affine data indices, enabling \tool to model most DNNs. 
%
%Another limitation is that 
Also, \tool does not support non-uniform tiling that maps a different number of data points to each PE. However, such mapping is also very rare because PEs are regular and load balancing is required across PEs.
%
%\HK{The following is now supported; will remove the paragraph but just wanted to let everyone know about the update}
%Finally, \tool does not support an accelerator with intermediate memory hierarchies other than two levels we target (Global L2 and Local L1 in each PE). We support only such memory hierarchies because they are the most common design in the recent accelerators~\cite{eyeriss_isca, parashar2017scnn, sharma2016high}.

==> tables/DSE-ExecutionTime_table.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
  
\begin{tabular} {|@{~} l @{~}|c|c|c|c|}
\hline
\multicolumn{1}{c}{\textbf{Dataflow}} &
\multicolumn{1}{c}{\textbf{Layer}} &
\multicolumn{2}{c}{\textbf{Results}} \\
\hline


%\multirow{3}{|*|}{\textbf{NVDLA and VGG16-CONV2}} 
\multirow{6}{*}{NVDLA} &
    \multirow{3}{*}{VGG16-CONV2} &
         & Execution time (minutes) & 12.20 \\
         & Number of design points & 175,861 \\
         & Effective DSE rate (Design points/sec) & 240.26 \\
    \multirow{3}{*}{VGG16-CONV11} &
         & Execution time (minutes) & 12.20 \\
         & Number of design points & 175,861 \\
         & Effective DSE rate (Design points/sec) & 240.26 \\


\hline
 \end{tabular}
  \caption{\small DSE statistics.}
  \label{table:dataflows}
\end{table*}



==> tables/DataFlow_table.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
  
\begin{tabular} {|@{~} l @{~}|p{2.5cm}|p{12cm}|}
\hline
\multicolumn{1}{|@{~} c @{~}|}{\textbf{Accelerator}} 
& \multicolumn{1}{@{~} c @{~}|}{\textbf{Dataflow Strategy}} 
& \multicolumn{1}{@{~} c @{~}|}{\textbf{Dataflow}} \\
\hline

Example for this work
& No Local Reuse (NLR)
& {\color{red} \tMap(1,1) \textbf{K} $\rightarrow$
  \tMap(Sz(R),1) \textbf{Y} $\rightarrow$
  \tMap(Sz(S),1) \textbf{X} $\rightarrow$
  \tMap(Sz(R),Sz(R)) \textbf{R} $\rightarrow$
  \tMap(Sz(S),Sz(S)) \textbf{S} $\rightarrow$
  \sMap(1,1) \textbf{C} } \\
\hline

%Checked
Example for this work
& Weight Stationary (WS)
& {\color{red} \tMap(1,1)         \textbf{K} $\rightarrow$
  \tMap(1,1)         \textbf{C} $\rightarrow$
  \tMap(Sz(R),3)         \textbf{Y} $\rightarrow$
  \sMap(Sz(S),1)         \textbf{X} $\rightarrow$
  \tMap(Sz(R),Sz(R)) \textbf{R} $\rightarrow$
  \tMap(Sz(S),Sz(S)) \textbf{S} } \\
\hline

%Checked
ShiDiannao~\cite{du2015shidiannao} 
& Output Stationary (OS)
& {\color{red} \tMap(1,1)         \textbf{K}    $\rightarrow$
  \tMap(1,1)         \textbf{C}    $\rightarrow$
  \tMap(Sz(R),Sz(R)) \textbf{R}    $\rightarrow$
  \tMap(Sz(S),Sz(S)) \textbf{S}    $\rightarrow$
  \tMap(Sz(R),1)     \textbf{Y}    $\rightarrow$
  \sMap(PEArrayWidth + Sz(S)-1, PEArrayWidth) \textbf{X}    $\rightarrow$  
  \Cluster(PEArrayWidth, P) $\rightarrow$
  \sMap(Sz(S), 1)    \textbf{X}   } \\ 
\hline

% Eyeriss logical PE
%Eyeriss~\cite{eyeriss_isca}
%& Row-stationary  
%& \tMap(1,1) \textbf{K} $\rightarrow$
%  \tMap(1,1) \textbf{C} $\rightarrow$
%  \tMap(1,1) \textbf{Y} $\rightarrow$
%  \Tile(R) \sMap(S,1) \textbf{X} $\rightarrow$
%  \Unroll \textbf{R} $\rightarrow$
%  \Unroll \textbf{S} \\
%\hline

% Eyeriss actual style; not logical PE
% Map entire row to a PE
Eyeriss~\cite{eyeriss_isca}
& Row-stationary (RS)
& {\color{red} \tMap(1,1)          \textbf{K} $\rightarrow$
  \tMap(2,2)          \textbf{C} $\rightarrow$
  \sMap(Sz(R),1)      \textbf{Y} $\rightarrow$
  \tMap(Sz(S),1)      \textbf{X} $\rightarrow$
  \tMap(Sz(R),Sz(R)   \textbf{R} $\rightarrow$
  \tMap(Sz(S),Sz(S)   \textbf{S} $\rightarrow$
  \Cluster(Sz(S), P)             $\rightarrow$
  \sMap(1,1)          \textbf{X} $\rightarrow$
  \sMap(1,1)          \textbf{S} } \\
\hline

%tMap (1,1) K
%tMap (1,1) C
%tMap (3,1) Y
%sMap (1,1) X
%tile (3) X
%unroll R
%unroll S

%C-brain~\cite{song2016c} 
%& Kernel-partitioning
%& \tMap(1,1)       \textbf{K} $\rightarrow$
%  \tMap(1,1)       \textbf{C} $\rightarrow$
%  \tMap(ks,ks)     \textbf{Y} $\rightarrow$
%  \tMap(ks,ks)     \textbf{X} $\rightarrow$
%  \Tile(ks) \sMap(ks,ks) \textbf{R} $\rightarrow$
%  \Tile(ks) \sMap(ks,ks) \textbf{S} \\
%\hline

%MAERI~\cite{kwon2018maeri}
%& OS in top clusters (virtual neurons), WS in PEs (multiplier switches)
%& \tMap(1,1)         \textbf{C} $\rightarrow$
%  \Cluster(Sz(R)))              $\rightarrow$ 
%  \sMap(1,1)         \textbf{K} $\rightarrow$
%  \tMap(Sz(R),1)     \textbf{Y} $\rightarrow$
%  \tMap(Sz(S),Sz(S)) \textbf{X} $\rightarrow$
%  \tMap(Sz(S),Sz(S)) \textbf{S} $\rightarrow$
%  \Cluster(Sz(S)))              $\rightarrow$ 
%  \sMap(1,1) \textbf{X}
%  \sMap(1,1) \textbf{S}  \\ 
%\hline

NVDLA~\cite{nvdla}
& Weight Stationary 
& {\color{red}
  \sMap(1,1)          \textbf{K} $\rightarrow$
  \tMap(64,64)        \textbf{C} $\rightarrow$
  \tMap(Sz(R),Sz(R))  \textbf{R} $\rightarrow$
  \tMap(Sz(S),Sz(S))  \textbf{S} $\rightarrow$
  \tMap(Sz(R),1)          \textbf{Y} $\rightarrow$
  \tMap(Sz(S),1)          \textbf{X} $\rightarrow$
  \Cluster(64) $\rightarrow$
  \sMap(1,1)          \textbf{C} } \\
\hline

 \end{tabular}
  \caption{\small A list of dataflows with description based on dataflow directives introduced in ~\autoref{subsec:dataflow-directives} and corresponding accelerators. \color{red} Sz(dim) denotes the size of corresponding layer dimension. For accelerators with a fixed number of PEs, we release the parallelism at the top level of clusters. In each cluster, omitted directives are inherited as \tMap from the upper cluster. We select free-variable mapping size (e.g., K and C dimension in Eyeriss). 
  %Some parameters such as the cluster size of NVDLA dataflow are co-optimized with hardware design parameters, thus they follow hardware design parameters. We mark such parameters using "P" followed by their names. Also, some mapping sizes such as the mapping size of K in Eyeriss dataflow is not specified thus free-variables. We select such free-variables to be minimum in this work.
  \vspace{-5mm} }
  \label{table:dataflows}
\end{table*}



==> tables/DataReuse_table.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
                     & \textbf{Temporal reuse}                                                                                    & \textbf{Spatial reuse}                                                                           & \textbf{Spatio-temporal reuse}                                                                                    \\ \hline
\textbf{Definition}  & \begin{tabular}[c]{@{}c@{}}Repeated access to a data \\ point over time in the same PE\end{tabular}        & \begin{tabular}[c]{@{}c@{}}Simulatenous access to a data\\ point over different PEs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Access to a data point from \\ different PEs over time\end{tabular} \\ \hline
\textbf{Implication} & Implies a stationary data class                                                                            & \begin{tabular}[c]{@{}c@{}}Implies opportunities \\ for multi-casting\end{tabular}               & \begin{tabular}[c]{@{}c@{}}Implies opportunities for \\ local forwarding among PEs\end{tabular}                   \\ \hline
\textbf{HW Requirement}  & \begin{tabular}[c]{@{}c@{}}Requires enough size of scratch \\ pad buffers for stationary data\end{tabular} & \begin{tabular}[c]{@{}c@{}}Requires NoC support \\ for multi-casting\end{tabular}                & \begin{tabular}[c]{@{}c@{}}Requires NoC support for \\ local forwarding\end{tabular}                              \\ \hline
\textbf{Benefits}    & \begin{tabular}[c]{@{}c@{}}Reduces number of accesses \\ to L2 and DRAM\end{tabular}                       & \begin{tabular}[c]{@{}c@{}}Reduces L2 to L1 \\ traffic on the NoC\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}Reduces L2 to L1, and\\  L1 to L2 traffic on the NoC\end{tabular}                      \\ \hline
\textbf{Example}     & \begin{tabular}[c]{@{}c@{}}Weights in weight-stationary \\ dataflow of NVDLA~\cite{nvdla}\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}Inputs in weight-stationary \\ dataflow of NVDLA~\cite{nvdla}\end{tabular}         & \begin{tabular}[c]{@{}c@{}}Partial-sum accumulation \\across PEs in Eyeriss~\cite{eyeriss_isca}\end{tabular} \\ \hline
\end{tabular}
\label{tab:data-reuse-summary}
\caption{Summary of data reuse opportunities across dataflows.\PC{Jun, What are your thoughts? Do we add origin as well as an another row?}\TK{This looks great. I think a row on origin, if possible, will also be useful.}}
\end{table*}


==> tables/DesignPoints_table.tex <==
\begin{table}[]
\begin{tabular}{|p{2cm}|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{Design Point} & \multirow{2}{*}{\# PEs} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}NoC bandwidth\\ (Data pts. per cycle)\end{tabular}} & \multicolumn{2}{l}{Spatial Reuse Support} & \multirow{2}{*}{Temporal Reduce Support} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Throughput\\ (MACs/Cycle)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Energy\\ (X MAC energy)\end{tabular}} \\
 &  &  & Multicast & Reduction &  &  &  \\
Throughput-Opt & 56 & 64 & Yes (Fan-out) & Yes (Fan-in) & Yes (Buffer) & 123.704 & 5.26 x 10$^9$ \\
 &  &  &  &  &  &  & 
\end{tabular}
\caption{Table} 
\end{table}

==> tables/HW_Implication_table.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}

\begin{scriptsize}
\begin{tabular}
{|p{0.7cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{0.7cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
\multicolumn{7}{|@{~} c @{~}|}{\textbf{Spatial}} & \multicolumn{7}{|@{~} c @{~}|}{\textbf{Temporal}} \\
\hline
\multirow{2}{*}{\textbf{Map}} 
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Coupling}}
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Reuse Opportunity}}
& \textbf{Inner} 
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Coupling}} 
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Reuse Opportunity}}  \\  \cline{2-7}  \cline{9-14}

& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}} 
& \textbf{Map}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}} \\
\hline
\hline

\multirow{3}{*}{K} &  \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{ } & \multirow{3}{*}{\ding{51}} &  \multirow{3}{*}{ } & \multirow{3}{*}{Multicast} & \multirow{3}{*}{ } & C & \ding{51} & \ding{51} &  &  &  & Reduction \\ \cline{8-14}
& & & & & & & R/S & \ding{51} &  & \ding{51} &  & Multicast &  \\ \cline{8-14}
& & & & & & & X/Y &  & \ding{51} & \ding{51} & Multicast &  &  \\ \hline
\hline

\multirow{3}{*}{C} &  \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{ } &  \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{Reduction} & K & \ding{51} & & \ding{51} &   & Multicast &  \\ \cline{8-14}
& & & & & & & R/S &  \ding{51} & & \ding{51} &  & Multicast &   \\ \cline{8-14}
& & & & & & & X/Y &  & \ding{51} & \ding{51} & Multicast &   &   \\ \hline
\hline

\multirow{3}{*}{R/S} &  \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{ } & \multirow{3}{*}{\ding{51}} &  \multirow{3}{*}{ } & \multirow{3}{*}{Multicast} & \multirow{3}{*}{ } & K & \ding{51} & & \ding{51} &   & Multicast &   \\ \cline{8-14}
& & & & & & & C & \ding{51} & \ding{51} &  &  &  & Reduction \\ \cline{8-14}
& & & & & & & X/Y &  & \ding{51} & \ding{51} & Multicast &   &   \\ \hline
\hline

\multirow{3}{*}{X/Y} &  \multirow{3}{*}{ } & \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{\ding{51}} &  \multirow{3}{*}{Multicast} & \multirow{3}{*}{ } & \multirow{3}{*}{ } & K & \ding{51} & & \ding{51} &   & Multicast &   \\ \cline{8-14}
& & & & & & & C & \ding{51} & \ding{51} &  &   &   & Reduction \\ \cline{8-14}
& & & & & & & R/S & \ding{51} & & \ding{51} &  & Multicast &  \\ \hline
\end{tabular}
\end{scriptsize}
  \caption{\small Reuse opportunities based on spatially-mapped dimensions in combination with innermost temporally-mapped dimensions. Filters (F), Inputs (I) and Outputs (O) are considered separately. For brevity, X/Y should be interpreted as X'/Y' as appropriate.}
  \label{table:reuse_opportunities}
\end{table*}



\begin{comment}
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}

\begin{scriptsize}
\begin{tabular}
{|p{0.7cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{0.7cm}|p{0.3cm}|p{0.3cm}|p{0.3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
\multicolumn{7}{|@{~} c @{~}|}{\textbf{Spatial}} & \multicolumn{7}{|@{~} c @{~}|}{\textbf{Temporal}} \\
\hline
\multirow{2}{*}{\textbf{Map}} 
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Coupling}}
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Reuse Opportunity}}
& \textbf{Inner} 
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Coupling}} 
& \multicolumn{3}{|@{~} c @{~}|}{\textbf{Reuse Opportunity}}  \\  \cline{2-7}  \cline{9-14}

& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}} 
& \textbf{Map}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{F}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{I}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{O}} \\
\hline
\hline

\multirow{3}{*}{K} &  \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{ } & \multirow{3}{*}{\ding{51}} &  \multirow{3}{*}{ } & \multirow{3}{*}{Distribution} & \multirow{3}{*}{ } & C & \ding{51} & \ding{51} &  &  &  & Reduction \\ \cline{8-14}
& & & & & & & R/S & \ding{51} &  & \ding{51} &  & Distribution &  \\ \cline{8-14}
& & & & & & & X/Y &  & \ding{51} & \ding{51} & Distribution &  &  \\ \hline
\hline

\multirow{3}{*}{C} &  \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{ } &  \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{Reduction} & K & \ding{51} & & \ding{51} &   & Distribution &  \\ \cline{8-14}
& & & & & & & R/S &  \ding{51} & & \ding{51} &  & Distribution &   \\ \cline{8-14}
& & & & & & & X/Y &  & \ding{51} & \ding{51} & Distribution &   &   \\ \hline
\hline

\multirow{3}{*}{R/S} &  \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{ } & \multirow{3}{*}{\ding{51}} &  \multirow{3}{*}{ } & \multirow{3}{*}{Distribution} & \multirow{3}{*}{ } & K & \ding{51} & & \ding{51} &   & Distribution &   \\ \cline{8-14}
& & & & & & & C & \ding{51} & \ding{51} &  &  &  & Reduction \\ \cline{8-14}
& & & & & & & X/Y &  & \ding{51} & \ding{51} & Distribution &   &   \\ \hline
\hline

\multirow{3}{*}{X/Y} &  \multirow{3}{*}{ } & \multirow{3}{*}{\ding{51}} & \multirow{3}{*}{\ding{51}} &  \multirow{3}{*}{Distribution} & \multirow{3}{*}{ } & \multirow{3}{*}{ } & K & \ding{51} & & \ding{51} &   & Distribution &   \\ \cline{8-14}
& & & & & & & C & \ding{51} & \ding{51} &  &   &   & Reduction \\ \cline{8-14}
& & & & & & & R/S & \ding{51} & & \ding{51} &  & Distribution &  \\ \hline
\end{tabular}
\end{scriptsize}
  \caption{\small Reuse opportunities based on spatially-mapped dimensions in combination with innermost temporally-mapped dimensions. Filters (F), Inputs (I) and Outputs (O) are considered separately. For brevity, X/Y should be interpreted as X'/Y' as appropriate. }
  \label{table:reuse_opportunities}
\end{table*}
\end{comment}


\begin{comment}

\begin{tabular}
{p{0.5cm}|p{1cm}|p{1cm}|p{2.5cm}|p{1.5cm}|p{0.5cm}|p{0.5cm}|p{1cm}|}
\hline
\multicolumn{1}{|@{~} c @{~}|}{\textbf{Dataclass}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{S-Dim.}}
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{S-Cpl}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{IMT-Dim.}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{T-Cpl}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{SR}} 
& \multicolumn{1}{|@{~} c @{~}|}{\textbf{TR}} \\
\hline
\hline

\multirow{10}{*}{Filter} 
& \multirow{2}{*}{K} & \multirow{2}{*}{CP} & (Y|Y')|(X|X') & DC & - & TD \\
& & & C|R|S & CP & - & - \\
 & \multirow{2}{*}{C} & \multirow{2}{*}{DC} & (Y|Y')|(X|X') & DC & - & TD  \\
& & & K|R|S & CP & - & -  \\
 & \multirow{2}{*}{Y/X} & \multirow{2}{*}{DC} & (Y|Y')|(X|X') & DC & FSD & TD  \\
& & & K|R|S & CP & FSD & -  \\
 & \multirow{2}{*}{Y'/X'} & \multirow{2}{*}{DC} & (Y|Y')|(X|X') & DC & FSD & TD  \\
& & & K|R|S & CP & FSD & -  \\
 & \multirow{2}{*}{R/S} & \multirow{2}{*}{DC} & (Y|Y')|(X|X') & DC & - & TD  \\
& & & K|(S|R) & CP & - & -  \\
\hline

\multirow{10}{*}{IfMap} 
& \multirow{2}{*}{K} & \multirow{2}{*}{DC} & R|S & DC & FSD & TD \\
& & & C|(Y|Y')|(X|X') & CP & - & - \\
 & \multirow{2}{*}{C} & \multirow{2}{*}{DC} & K|R|S & DC & - & TD  \\
& & & C|(Y|Y')|(X|X') & CP & - & -  \\
 & \multirow{2}{*}{Y/X} & \multirow{2}{*}{CP} & K|R|S & DC & PSD & TD  \\
& & & C|(Y|Y')|(X|X') & CP & PSD & -  \\
 & \multirow{2}{*}{Y'/X'} & \multirow{2}{*}{CP} & K|R|S & DC & PSD & TD  \\
& & & K|R|S & CP & PSD & -  \\
 & \multirow{2}{*}{R/S} & \multirow{2}{*}{DC} & K|(S|R) & DC & FSD & TD  \\
& & & C|(Y|Y')|(X|X') & CP & PSD & -  \\
\hline

\multirow{10}{*}{OfMap} 
& \multirow{2}{*}{K} & \multirow{2}{*}{CP} & C|R|S & DC & - & TR \\
& & & (Y|Y')|(X|X') & CP & - & TR \\
 & \multirow{2}{*}{C} & \multirow{2}{*}{DC} & R|S & DC & SR & TR  \\
& & & K|(Y|Y')|(X|X') & CP & SR & TR  \\
 & \multirow{2}{*}{Y/X} & \multirow{2}{*}{CP} & C & DC & SR & TR  \\
& & & K|((Y|Y')|(X|X')) & CP & SR & -  \\
 & \multirow{2}{*}{Y'/X'} & \multirow{2}{*}{DC} & C & DC & - & TR  \\
& & & K|((Y|Y')|(X|X')) & CP & - & -  \\
 & \multirow{2}{*}{R/S} & \multirow{2}{*}{CP} & C & DC & SR & TR  \\
& & & K|((Y|Y')|(X|X')) & CP & SR & -  \\
\hline
\hline
 \end{tabular}
  \caption{\small A summary of possible spatial (SR) and temporal reuse (TR) opportunities based on spatially mapped (S-Dim) and inner-most temporally mapped (IMT-Dim) dimensions. S- and T-Cpl represents the coupling of the S-Dim and IMT-Dim with the data class in the left-most column. FSD, PSD, SR, TD, and TR are full spatial distribution, partial spatial distribution, spatial reduction, temporal distribution, and temporal reduction, respectively.}
 \end{comment}
